"Is Reporting Worth the Sacrifice of Revealing What I Have Sent?": Privacy Considerations When Reporting on End-to-End Encrypted Platforms

User reporting is an essential component of content moderation on many online platforms -- in particular, on end-to-end encrypted (E2EE) messaging platforms where platform operators cannot proactively inspect message contents. However, users' privacy concerns when considering reporting may impede the effectiveness of this strategy in regulating online harassment. In this paper, we conduct interviews with 16 users of E2EE platforms to understand users' mental models of how reporting works and their resultant privacy concerns and considerations surrounding reporting. We find that users expect platforms to store rich longitudinal reporting datasets, recognizing both their promise for better abuse mitigation and the privacy risk that platforms may exploit or fail to protect them. We also find that users have preconceptions about the respective capabilities and risks of moderators at the platform versus community level -- for instance, users trust platform moderators more to not abuse their power but think community moderators have more time to attend to reports. These considerations, along with perceived effectiveness of reporting and how to provide sufficient evidence while maintaining privacy, shape how users decide whether, to whom, and how much to report. We conclude with design implications for a more privacy-preserving reporting system on E2EE messaging platforms.

==> sections/04_findings_trial.tex <==
\section{Findings}
\subsection{E2EE platforms in reporting systems}
 We first described the role E2EE platforms play in reporting systems. We found that participants expect a limited view of the reported conversation, account information, and device information to be shared with platforms for moderation purposes. While participants believe platforms will further use data from user reports to develop better anti-harassment tools, mine usage patterns, or help legal investigations, they are also worried that data from user reports might be used to generate profiles for targeted advertisements or susceptible to malicious hackers due to insecure storage at rest by platforms.
 
\subsubsection{Data access of platforms}
\textbf{Messages.} Most participants believe that most E2EE messaging platforms have access to the reported message and the contextual messages around it, which they consider to be important for informed moderation decisions. As P3 described, \emph{``the context helps moderators understand what we've been discussing and where the abuse was being perpetrated or where it was taken place.''} Compared to social media platforms in general, E2EE platforms are believed to have more limited access to the context of the reported message. As P11 expressed, \emph{``E2EE platforms get access to that message and the context of that message as well as whatever else they would have to do on my account normally...the contextual might be less on an encrypted message platform.''}

However, some participants also expect E2EE platforms with the most stringent privacy principles to have no access to the context around the reported message or even the content of the reported message. These participants are also more privacy-conscious and opted to use these platforms after deliberation. P14 told us that \emph{``Signal can never see messages unless you send them a screenshot or something. So my preference would be that they have as little access as possible.''} These participants attribute their expectation to the E2EE platform's reputation for privacy protection: \emph{``if somebody finds out that this platform actually shares the last N messages or this entire chat, this press would be too much of a negative thing for the platform [P1].''}

\textbf{Metadata: account, device, and conversation information.} Nearly all participants think that, when they report a message, the platform has access to their account information (i.e., their phone number, email address, registration time, and history of reporting and being reported) and relevant conversation information (i.e., who you chatted with, when you chatted, how frequently you chatted with them). They also expect most E2EE platforms to have access to device information that does not require extra permissions from users, such as the battery level, model of the phone, and phone carriers. 

On the other hand, how much information is shared also varies across E2EE platforms. For example, P6 believes that platforms with centralized servers can collect more conversation information when relaying messages between ends, while platforms without centralized servers, such as Signal, collect only a little. As P4 said, \emph{``typically they only know when you last logged on and they typically don't even know who sent a message. Of course, they have to know who to deliver the message to. But as I understand, [Signal] knows almost nothing.''} 
 
Almost all participants are not concerned about sharing their metadata with the platform when reporting unwanted messages for the next two reasons. First, users have low privacy expectations about these kinds of information since most E2EE platforms do not explicitly guarantee the invisibility of metadata to third parties. In fact, most participants believe that platforms have already collected it before any user reporting. P13 expressed such an idea, \emph{``I'm not worried about sharing [metadata] when I report, because I've anyway shared all of this information with them by even using their application. So that information is already with them.''}

 %P1: Yeah, so this is mainly based on just how the existing end-to-end encryption platforms are run. I don't think they make any guarantees to keep this information private. Well, at least I know Telegram doesn't like, they don't say   your phone number is like, private. I don't think they guarantee that. So I would expect that probably they're going to share it and as a part of just interacting with the platform, like getting verification codes and that kind of stuff.
 
Second, while concerned about the sensitivity of metadata, some participants acknowledge its importance for reviewing user reports. For example, device information can be used to identify whether the sender uses a fake phone, or is a bot. As P6 expressed, \emph{``device information can be very useful and very identifying. I would like for them not to have it at all probably, but it can help to know if a person is using a fake phone or is using an Android VM and Virtual Box, if it's a bot spamming misinformation messages.''} Similarly, they believe that account information, especially the history of reporting and being reported, is important for reviewing their reports. P5 said: \emph{``So they need account information to sort of build a profile of that person to understand whether they constantly put in fake requests or they constantly report people and that sort of a thing.''}

\subsubsection{Data storage by platforms}
Participants expect that the data from user reports will be stored on the platform server for some time. How long the data will be stored depends on local legal requirements, and moderation requirements as moderators need data from previous user reports for future reference. P11 explained his expectations in detail: \emph{``because sometimes the abuse may not be enough to delete the account or ban it so I should be able to act on that information at a later date. I would also imagine for liability reasons they might be required to keep stuff for a certain amount of time.''}

Participants have mixed expectations about the protection of data from user reports by E2EE platforms. Despite acknowledging their limited understanding of technical details, some participants trust E2EE platforms to securely store the data at rest. P13 told us that \emph{``the trust I placed not fully based on understanding technical details, but in trusting them to do the security well.''} 
Other participants, who are more knowledgeable about secure practices, expressed concerns about the platforms' ability to protect the data from potential hacking. For example, P9 was worried that, while the data from reports may be encrypted in transit, it has to be decrypted for moderators' review and might not be encrypted at rest. Platforms may also fail to enforce strict access controls. One participant also expressed concerns that \emph{``even if they had the best intentions and wanted to provide encryption, they might do it for text, but not media, whether it's video or images [P13].''}

% P9: I don't want my device information to be associated with a pseudonym, for example. Why? Because that's a kind of doxing. So I wouldn't want a hacker to get access to that and possibly DOX me.

% P9: Not in particular. I mean, I understand they could have theoretical access to it. I'm more concerned with hackers intercepting banking logins or getting wholesale access to encrypted messages because the conversation and the social graph are the more exploitable things. I think in that regard, my personal information, sure, but my personal information is not really exposed as much here as it might be in another context, like banking or school,

\subsubsection{Data usage by platforms} \label{data usage}
\textbf{Anti-harassment tooling.} Some participants believe that data from user reports will be used to improve anti-harassment tools. Platforms can learn patterns of spurious links in reported messages and block reported accounts that send similar links more proactively. P13 expressed her hopes for this purpose: \emph{``But it's not a worry, it's actually a hope that they would use it towards understanding what issues users face better and trying to make it a safer platform just on the whole.''}

\textbf{Data mining.} Participants also envision that the platform may use the data from user reports to analyze usage patterns and inform its development priorities. For example, the platform can tell which operating systems users are using from device information and prioritize security measures on popular operating systems. The content of messages can reveal cultural interaction patterns as suggested by P14, \emph{``there's a lot of tension between religious groups in India---you can link to the language that they're using, try to see if there's an imbalance that needs to be considered in how you develop your platform strategy.''} Since the data are analyzed in aggregate, participants do not feel uncomfortable about data mining. 

\textbf{Legal investigation.} More than half of the participants believe that data from user reports might be relevant to the investigation of illegal acts (such as terrorism, intimate partner violence, and child abuse) and therefore would be requested by law enforcement agencies. For example, the device and account information of the reported person may help law enforcement agencies identify offenders, and the contextual messages in the reported conversation may also be direct evidence of illegal acts. P14 argued further that the history of user reports could be used to undermine testimony by describing the following example: \emph{``let's say a woman goes to the police and says this guy is stalking me...[by] sending me messages on this platform and waiting outside my house. [But the police] find that you haven't reported any of the messages, suggesting you don't really take it seriously.''}

\textbf{User profiling for targeted ads.} 
Participants have opposing views about whether platforms generate user profiles for ad targeting based on data from user reports. Some participants argue that it is technically and economically infeasible for platforms for two reasons. First, they note that personal information in reported conversations is less organized than the phone number or email address, and therefore platforms need to invest huge computational power, disproportional to the benefits they receive from advertisements, to 
extract personal information. Participants also believe that it is not a comprehensive way to profile users since \emph{``somebody has to either have reported or been reported, and I don't know what percentage of the users are in that group [P10].''}

Other participants believe that it is highly probable for platforms to profile users using data from reports. Platforms can build a granular social graph from conversation information, associate users' metadata with contact information, or even infer their preferences or identities. As P14 suggested, \emph{``if I'm reporting a bunch of homophobia, then the platform could infer that I'm gay with a high probability from that data.''}

Participants also respond with mixed feelings if they know E2EE platforms profit off of generating user profiles from their reports. People who have high privacy expectations about E2EE platforms expressed great disappointment, as P8 clearly stated, \emph{``The way I phrase it to people is your information is valuable, it's financially worth something and they're encouraging you to give them this valuable thing for free.''} In contrast, participants who use E2EE platforms because of peer influence are more indifferent, as P5 explained, \emph{``let's say even if WhatsApp is using that information, I'm already being profiled on so many other platforms that adding in this little thing wouldn't affect my day-to-day life as much.''}

% P4: I think it's more the principle of the thing. I think that big tech shouldn't be profiting off of my information. So it's not necessarily that I have something to hide, it's just I have nothing to share.

\subsection{Moderators in reporting systems}

\subsubsection{Data access of moderators}
Participants have a mixed understanding of the relationship between platform moderators and the platform. Some participants consider these two stakeholders as one entity, thereby believing that platform moderators have the same access as the platform to the information. For example, P2 told us that \emph{``I kind of bunch platform and platform moderators into one entity. I kind of already assume that they have that information because they work for the platform.''}

In contrast, other participants think that platform moderators have a lower level of access to data than the platform. We observe uncertainties among these participants about which subset of data is shared with platform moderators exactly. P5 described his uncertainty as follows, \emph{``To me, the platform knows everything, but I don't have a clear idea about where platform moderators lie in that spectrum of the amount of information that they can access.''} In the following, we discuss information that participants believe platform moderators may have less access to.

% P5: I think let's say I'm reporting a specific message. They might have access to all the messages, but initially they might just, let's say, look at a few messages that are around those reported messages, just for a little bit more context. And then they might make a decision. And if not, they might request more information or maybe it's available to them.

\textbf{Account information.}
A considerable number of participants think that platform moderators only have access to non-identifying account information, such as the registration time and history of reporting and being reported, but no personal identifiers like emails, phone numbers, or platform handles. For personal identifiers, participants believe that moderators will \emph{``see some kind of encrypted or hashed kind of version of that number, so they can tell different accounts apart, but they can't kind of reverse engineer who it is [P1].''}

The criteria that participants use to make this distinction is whether they think this piece of account information is important for moderators to make moderation decisions. As P5 has summarized clearly, \emph{``The way I'm thinking about [which information is shared] is what information do I need to make a decision about a specific reported message or a group chat or a person.''} He then gave an example: the history of reporting and being reported can be used to identify false reporters and frequent abusers, but \emph{``other account information isn't as revealing as these two pieces of information.''}
Even for the history of reporting and being reported, several participants expect that a platform that really cares about user privacy would only provide platform moderators with some derivative of this history, such as \emph{``the output of a classification algorithm acting on this information [P14].''}

\textbf{Device information.} Similarly, some participants also expect that only anonymized device information is shared with platform moderators, as evidenced by the words of P11, \emph{``I wouldn't think device information, at least nothing uniquely identifiable, but maybe iPhone or Android or something like that.''} Further, several participants also believe that platform moderators are only provided with some derivative of device information because they are not able to interpret device information on their own. P6 believed that \emph{``The platform would be able to [use device information to] track people across different applications, but the moderators themselves would not be able to use it to perform the tracking.''}

% \textbf{Relationship with the platform} More than half of participants believed that the platform has access to any reports made to community moderators in the sense that the platform automatically stores data of these reports. The overarching principle is summarized by P11 that \emph{"I feel like anything done on the platform is always going to be accessible to the platform beyond the single person who's doing it"}. That being said, participants do not think the platform will be \emph{" bothering themselves too much on a very low level about a specific report [P5]"}.
With a hierarchical structure of reporting systems on messaging platforms in mind, most participants believe that community moderators have access to less data than platform moderators when reviewing user reports. For example, some think that community moderators have access to a limited set of account information, such as the registration time and the location country. They may also only know the history of reports in the scope of their community. P11 implicitly made a distinction between the information community moderators should have versus platform moderators during the interview: \emph{``I'd be fine with a community moderator, for example, knowing how old my account is or maybe what country I'm logged in from, but not something like the email recovery address I use or my IP address. Seems like more of a platform moderator type of information.''}

Participants gave two arguments to explain this distinction. First, they think that community moderators are more knowledgeable about specific community norms and parties involved in the reported conversation than platform moderators. As a result, the platform provides platform moderators with more information to make up for their disadvantages, or equivalently, refrains from giving community moderators unnecessary access to more information. P5 explicitly talked about his perception of community moderators: \emph{``The way I think of community moderators is like a person within the community that's also sending messages and constantly an active participant in that community...They have enough context to just look at the messages and make a decision, rather than platform moderators who need more technical information to kind of detect this kind of thing.''}


Second, participants perceive that different groups of moderators are responsible for different kinds of user reports and therefore have access to different data. For example, participants believe that platform moderators are in more urgent need of device information to identify whether a reported message is spam. As P6 explained, \emph{``for community moderators, I would pull out the account information and the device information. That would be up to the platform to detect...if someone is a bot or spam person.''} Therefore, platform moderators are also more equipped to interpret device information, as evidenced by P5's words, \emph{``not all people might understand how to use that information within the community.''}

\subsubsection{To whom should I report?} \label{to whom report}
Whether moderators can make an effective and efficient decision to protect users' privacy greatly influences participants' decisions about whom they should report to. Participants think that the following three dimensions contribute to the variance between the effectiveness and efficiency of platform moderators and community moderators. 

\textbf{Moderation areas.} More than half of the participants believe that community moderators are more familiar with \textit{community norms} and therefore can better detect disrespectful behaviors, while platform moderators are more knowledgeable about \textit{platform policies} and can better identify reports of illegal behaviors. P1 explicitly talked about this contrast: \emph{``My mental model of reporting to community moderators is more of a personal issue like [complaints that] `I don't like what's being posted'; my mental model of reporting to platform moderators is more of an illegal stuff like posting child pornography, which violates platform rules.''} 

Therefore, participants tend to report to moderators who they believe can quickly identify the abusiveness of their report and take swift action to protect their privacy. P7 explained his reasoning to us: \emph{``[Abusers] have the potential to do doxxing type activities. So I would want some quick action and it's clearly against stated platform policies. So I would want the platform to take quick action.''}

\textbf{Moderation actions.} Most participants think that platform moderators can delete messages or ban accounts from chat and delete accounts from the platform, while community moderators can do everything but delete accounts from the platform. Hence, participants tend to report to platform moderators if they expect only deleting the abuser's account from the platform can prevent further dissemination of their personal information, as P3 described, \emph{``I believe [platform moderators] are the ones that could solve this problem because I don't need any of these words to be removed and feel the particular account should be deactivated and permanently deleted from the platform.''}

% P4: Platform moderator. And yeah, platform moderator immediately. I would try to go as high up as possible. Higher possible? Is that because could you explain that? Why higher as possible? Yeah. Because this person has just made an actual threat that could become risky to me.

\textbf{Time and resources.} Several participants also believe that community moderators have more time and resources to review user reports than platform moderators. As a result, participants may report to community moderators if they expect more efficient moderation actions to protect their privacy. P6 observed that \emph{``I'll say there are way more community moderators than platform moderators. And also during the time of the night and weekend hours, they would probably be able to moderate while platform moderators are out of duty.''}\\

On the other hand, participants are also concerned that platform or community moderators might abuse the personal information in their reports, such as taking sides with the abuser, leaking information, or doxxing the reporting person. However, a majority of participants have more trust in platform moderators than community moderators to not be abusive or privacy-violating for the following reasons.

\textbf{Expertise.} First, almost all participants perceive platform moderators as more professional in reviewing user reports and trained on how to protect users' privacy. Therefore, platform moderators are believed to recognize the sensitivity of personal information, adhere to codes of conduct about how to access and share information, and refrain from making biased decisions from their personal standpoints. In contrast, as P6 described, \emph{``community moderators are a person voted by the public and probably not versed in privacy and could abuse that information to track down people.''}

\textbf{Accountability.}
Second, many participants think platform moderators are more consistently accountable for potential abuse than community moderators. Platform moderators are supervised by the platform, thus there are more consequences if they violate users' trust; for example, \emph{``getting fired or losing health insurance [P11].''} In contrast, the accountability of community moderators varies across communities. Community moderators who are invested in communities care about their reputation and \emph{``they would have more to lose by losing their reputation and their ability to use the platform [P9],''} while community moderators in a workplace might only be loyal to \emph{``human resources or the management rather than the users and the community itself [P9].''} 

\textbf{Personal connections.}
Moreover, participants also believe that community moderators are more likely to have personal connections with the reporting or the reported person and have motivations to misuse personal information in the reports. P6 gave an example: \emph{``if [community moderators] don't like someone in the chatroom, might do harm with the information with the advantage they possess over some people.''} In comparison, platform moderators are perceived to be distant and unlikely to take a personal grudge against users.

\textbf{Time and resources.}
While having more moderation time and resources can be a motivator for people to report to community moderators, participants also believe that it increases the chances that community moderators might notice the personal information in users' reports and take advantage of it. P4 clearly expressed his concerns: \emph{``I'm assuming that the scope [of community moderators] is smaller and they're responsible for moderating fewer people. My concern would be that they have more time to be worried about me, or they have more time to actually think about this one report.''}

% P11: But generally, if I'm reporting other users and I'm reporting stuff that they sent, I'm not as concerned about that because of the context. But yeah, generally speaking, I would rather have reports to go to community moderators because I think that they have less access in general and they're more likely to be invested in or concerned about the general health of that community that they're moderation than the platform moderator would be.


\subsection{Privacy considerations about user reporting on E2EE platforms}

\subsubsection{Whether I should report?} \label{whether report}
We observed that participants compare the privacy risks of reporting with the protection the report can provide to decide whether they should report, as P4 summarized, \emph{``the question is, is reporting this message or this person worth the sacrifice of revealing whatever I've sent.''} For instance, participants tend to report abusive messages if they are in a group chat but tend not to if in a direct message (DM). P2 explained her reasoning in detail: \emph{``For a DM, I don't have to risk myself being identified [by moderators] because of the photo if I don't want to see the photo anymore...I can just delete it on my end and I won't have to see it. But if it's a group chat, then if I delete it on my end, other people can still see it and I don't want other people to still see it. That's why I have to take the risk to report them and have the photo deleted.''}

\textbf{Ineffectiveness.} However, reporting is not always effective in protecting users’ privacy, especially when abusers have already had access to their personal information. For example, when personal photos are used in abusive messages, taking down the photos from the chat cannot prevent further dissemination since abusers can take screenshots or download the photos, and banning the abuser from chat may even motivate them to share photos in more chats or on other platforms. Similarly, when abusers weaponize people's address or phone number to make threats, participants chose not to report to the platform because \emph{``[the most] the platform can do is to probably remove the particular user from the account, but at end of the day from the chats, [the abuser] could already note down my home address [and] compromise my security [P3].''}


% P11: [personal photos] But there's some degree to which I've already lost control of that situation. However, it would be important for me to report it to the moderators anyway, because it might prevent that user from doing that to other users in the future.

% P4: I'm expecting moderators to delete the edited photo at the bottom. I see. And I yeah, it's probably useful to have it on record that this person has sent a harassing message.

\textbf{Inefficiency.} In addition to effectiveness, the efficiency of moderation actions also influences people's decisions to report. When abusers send personal photos of victims in a group chat, P11 explained his consideration to us: \emph{"it's really a question of time ... maybe there's fewer extra people know if I got the message deleted fast enough, but I would have to assume that the community moderators would be very fast to do that.''} 


% P10: Right. So if I report it, then it's unclear to me if I'm actually going to be more protected, if they'll actually somehow I don't know what they would do, like, somehow get this person and not harass me or send me threats. But then at the same time, I don't know if that information just gets stored somewhere.

% P10: I think what it would come down to for me is what are the risks of not reporting this? And then I also want to know what will happen if I do report it. Like, what meaningful sort of action will take place if this is just going to be some log in this platform's storage and they're just going to be like, yeah, we know that on this day, at this time, this person sent this abusive message. In the short term, that doesn't really do anything to protect me. Maybe it contributes in some way to a safer platform. So I think I would be weighing these trade offs.
\textbf{Privacy risks of reporting.} Participants are also concerned about the privacy risks of reporting; for instance, if there is extremely sensitive information in the conversation that would then be shared with moderators. It could be sensitive political views, intimate photos (used in cases of non-consensual intimate imagery), or personally identifying information (e.g., home address, social security number).

% P11: But that is something that would prevent me from making a report if I knew that they would gain access to everything in the group chat. Chances are if I'm using Platform, I probably am using that for some specific privacy reason. It would kind of defeat the purpose of using the platform.


\subsubsection{Which information should I share?} \label{which report}
As we have discussed in \S~\ref{platform - data access}, participants are more concerned about disclosing to moderators the content of their conversations than their account and device information when reporting unwanted messages. In the following, we describe how participants carefully decide which information in their conversation they want to share with moderators to both provide evidence against abusers and protect their own privacy.

\textbf{Towards making an informed moderation decision.} Participants are willing to share information that they believe is important for an informed and fair moderation decision. More than half of the participants chose to share the context around the reported message with moderators to both underline the abusiveness of the reported person and to show their own innocence. For example, P13 suggested that abusive messages can be contextual: \emph{``Sometimes the hate speech can be sarcasm and mockery. It can seem unoffensive when out of context, but with the context, it might make more sense,''} whereas P4 tried to show his civility: \emph{``The other person in this chat is definitely being abusive. But my concern is that if I don't share my own messages, then from the perspective of moderators, I could have also said something horrible.''} 

% P4: Yes, because I think the context is important. And I think if I don't report all of them, then it could look like I'm trying to hide something. It could look like I'm also sending abusive messages. And if I report everything, it shows that I at least made an attempt to be civil.

However, participants tend to share less information and select less sensitive information as long as they believe what they are sharing is enough for an informed and fair moderation decision. For instance, several participants choose not to share the context around the reported message because they believe the reported messages are abusive on the surface and \emph{``the other context might not really help in this position [P3].''} When receiving abusive messages repeatedly, participants choose to only report the abusive messages that do not include their personal information. P2 decided not to report the abusive photo of her: \emph{``Because the whole point of getting this person reported is to have the messages deleted and then banned. And based on the first two [abusive messages without photos], I think it's pretty obvious some action will be taken.''}

% \outline{hope other metadata can help here}
% P5: I guess, for instance, if this person is like a repeat offender, they might see in the history if this person has been like yeah, I think that's one of the metadata that helps them understand whether it's a repeat offender or not.

% P5: [personal photos: not share his personal photos]  I do agree that this definitely might weaken my acquisition, but I think all the metadata that they might have would eventually help them make an informed decision. But I do agree that my acquisition would be weakened if I don't share the whole chat and the photographs.

\textbf{Less willing to share identifying information.} In general, participants feel less comfortable sharing with moderators messages containing personally identifying information (e.g., phone number, email address, workplace) than those containing information about personal preferences. P4 compared these two kinds of information as follows: \emph{``I think a platform moderator is probably not interested in my personal life. But if I'm revealing where I live, contact information, or my workplace, that would concern me more.''} This is because participants believe identifying information, once put together with information about personal preferences, opens the way for greater abuse, as P10 explained, \emph{``if I make a comment about my political views and it's not attached to any identifier, then you can't trace it back to me and I'm not really concerned about that.''} 

As a result, if participants are certain that their reports are anonymized to platform moderators, they are willing to share more contextual information due to the belief that moderators can not easily associate their personal preferences with their identity. For example, in cases when platform moderators only have access to anonymized reports, P2 told us: \emph{``I'm comfortable sharing the entire chat. But if they have access to my email, to my phone number, to linked social media, then I wouldn't be comfortable sharing all of it.''}

On the other hand, participants are less willing to share information about personal preferences (e.g., medical history, personal photos, political views) with community moderators. In their mental models, participants perceive platform moderators as \emph{``in a far, far away location and removed from the applications infrastructure [P13]''} but community moderators as someone they might run into in their personal life. Therefore, disclosing personal preferences to community moderators not only introduces the risk of abuse but also feels to participants more awkward and confrontational. When receiving abusive messages with his intimate photos, P11 clearly expressed his concerns about context collapse: \emph{``The concern is that when people see the photos you change their impression in some way. [So] I would prefer platform moderators than who I have some relationship with, even if it's in a vague sense that they moderate the community...I'd rather it not be someone who has any ties to me at all.''}
